Transform-Dependent Adversarial Attacks

Deep networks are highly vulnerable to adversarial attacks, yet conventional attack methods utilize static adversarial perturbations that induce fixed mispredictions. In this work, we exploit an overlooked property of adversarial perturbations--their dependence on image transforms--and introduce transform-dependent adversarial attacks. Unlike traditional attacks, our perturbations exhibit metamorphic properties, enabling diverse adversarial effects as a function of transformation parameters. We demonstrate that this transform-dependent vulnerability exists across different architectures (e.g., CNN and transformer), vision tasks (e.g., image classification and object detection), and a wide range of image transforms. Additionally, we show that transform-dependent perturbations can serve as a defense mechanism, preventing sensitive information disclosure when image enhancement transforms pose a risk of revealing private content. Through analysis in blackbox and defended model settings, we show that transform-dependent perturbations achieve high targeted attack success rates, outperforming state-of-the-art transfer attacks by 17-31% in blackbox scenarios. Our work introduces novel, controllable paradigm for adversarial attack deployment, revealing a previously overlooked vulnerability in deep networks.

==> archive/conclusion.tex <==
% \section{Discussion}


% To the best of our knowledge, this is the first work to demonstrate that a single (imperceptible) adversarial perturbation can be used to trigger transform-dependent (controllable) attacks. The idea is simple but reveals new and intriguing properties of adversarial attacks and vulnerable spaces in deep networks. 
% %
% For instance, this method can be viewed as a simple alternative to backdoor attacks. But unlike standard backdoor attacks~\cite{gu2019badnets, xu2023batt}, which require to attack in the way that training a backdoor model with malicious triggers, instead, we add a single perturbation that with image transformations can trigger (desired) responses from the models. Here, we provide additional properties and experimental discussions on transform-dependent attacks.




% % \subsection{Transform-dependent attacks study}
% % \subsection{Independent attacks across transforms}

% % \label{subsec:study}
% % \input{figures/fig-trend}

% % \noindent\textbf{Number of transformations.} 
% % Since we can embed multiple targeted attacks by transforming a single perturbation, a natural question to ask is \textit{``how many transform-dependent targets can we embed in one attack?''}
% % To answer this question, we conduct a study on \{ResNet50, InceptionV3, ViT-L-16\} with scaling, blurring, gamma correction, and JPEG compression.
% % %
% % We initialize the transform parameter sequence $\{\theta_i\}$ as $\{0.5\}$ for scaling, blurring, gamma correction, and $\{20\}$ for JPEG compression for the first attack. {Then we append new $\theta_i$ samples to the transform sequence by adding an adaptive step size to the $\text{max}\{\theta_i\}$, performing new transform-dependent attacks with the new sequence until $\{\theta_i\}$ has a maximum of 25 samples with $\text{max}\{\theta_i\}$ 1.5 for scaling and blurring, 2 for gamma correction, and 80 for JPEG.}
% % %
% % We assign a different target label for each sample from the dataset label space at random.
% % %
% % ASR vs number of samples in~\cref{fig:attack-trend} shows ASR drops as the number of samples increases. This indicates that the difficulty of transform-dependent attacks increases as we attempt to embed more targeted attacks in a single perturbation through image transformation. While each curve shows a downward trend, the rates of decline differ significantly for different models and transforms. Among all four transforms, scaling and JPEG have a larger capacity for embedding more targeted attacks compared to blurring and gamma correction. Overall, among all three models, ResNet50 has the largest embedding space, while ViT-L-16 has the smallest.

% \noindent \textbf{Memory and computation resources. } We used a single {NVIDIA RTX 2080Ti (12 GB)} for all the experiments. Average times for generating $3$-target attacks are $2.61$ sec/image.

% % \Salnote{Fix eps to 8 ?}
% % \input{tables/supp/tab-cls-adapt}

% % \noindent\textbf{Adapt other optimization methods.} 
% % We primarily focus on solving transform-dependent attacks using PGD~\cite{madry2017towards}, an iterative method for solving adversarial attack optimization problems. In principle, our attack formulation can also be generated with other optimization methods. Here, we provide additional results of our attacks adapted using some commonly used methods, including single-step FGSM~\cite{goodfellow2014explaining}, iterative MIM~\cite{dong2018boosting}, and loss modification C\&W~\cite{carlini2017towards}, and compare these results to those obtained with PGD presented in \cref{tab:cls-asr}. Results in \cref{tab:attack-adapt} show that the iterative methods MIM, C\&W, and PGD are more effective than the single-step FGSM in achieving higher ASRs.



% \noindent \textbf{Limitations.} 
% While our work provides important empirical demonstrations of transform-dependent adversarial attacks across various settings, there remain several limitations that warrant further investigation. Firstly, although we observe the effectiveness of these attacks in inducing diverse misclassifications through input transformations, the underlying mechanisms by which the adversarial perturbations interact with and manipulate the transformations to change network behavior are not fully clear. A deeper feature-level study is needed to understand how different transformations modify the input content or frequency components in ways that can be exploited adversarially.
% Secondly, while we showcase real-world implications through the object detection task, the deployment of such transform-dependent attacks in physical environments and their effectiveness under real-world conditions requires more extensive evaluation. 

% \noindent \textbf{Future directions.} 
% Based on the limitations of this work, we identify several future directions, including feature-level analysis to gain insights into how image transformations introduce or modify content properties that enable adversarial manipulation when combined with carefully crafted perturbations. Additionally, extending the transform-dependent formulation to patch-based attacks tailored for physical environments, where localized adversarial patterns can induce diverse effects by transforming the camera viewpoint or object pose, rotations, and locations, is another promising direction. Our proposed attack generates a ``static/fixed" perturbation that can trigger ``dynamic/controllable" adversarial effects in real-time deployment. 
% While the computational cost for generating such adversarial perturbations is proportional to the number of attacks, different attacks can be deployed or changed with minimal cost through simple transformations. 
% For instance, in surveillance systems or facial authentication, an attacker could hide or impersonate a person by simply transforming the input image. In principle, this method can be extended to physical attacks where attackers manipulate objects through simple transformations like scaling and rotating to achieve different effects. For example, an object can be made to appear, disappear, or be misclassified based on distance or blur.


\section{Conclusion}
\label{sec:conclusion}
This work unveils transform-dependent adversarial attacks, a formidable new threat where carefully crafted perturbations can induce a wide variety of targeted misclassifications by dynamically transforming the input. Our extensive experiments across diverse models and tasks demonstrate the remarkable vulnerability of deep networks to manifest controllable attack effects from a single perturbation. These attacks shatter the traditional notion of adversarial inputs being static, isolated instances - their adversarial nature is now a complex, chameleon-like capability to react differently under transformations. This work calls for a necessary paradigm shift in how we understand and defend against adversarial threats in machine learning.


==> archive/experiment.tex <==
\section{Experiments}
\label{sec:experiment}
In this section, we present the main results of transform-dependent adversarial attacks. We begin with image classification and demonstrate that our attack formulation is highly effective across a wide range of transforms, applicable to various architectures. Additionally, our analysis of transform-dependent attacks in blackbox and defended model scenarios shows that they achieve comparable performance to state-of-the-art methods specifically designed for blackbox transferability. We further highlight the generalizability of our attack formulation to object detection, emphasizing its practical applicability and potential use cases.


\input{tables/tab-cls-asr-range}
\input{figures/fig-loss}


\subsection{Experiment setup}
\noindent\textbf{Models and dataset.} 
We utilize pretrained image classification models from Pytorch Torchvision \cite{paszke2017automatic}, which provides models pretrained on ImageNet dataset~\cite{deng2009imagenet} for a variety of families and architectures. Models are trained with data augmentation techniques including random cropping, rotation, flipping, and color jittering, so that they align with our assumption in \cref{eq:transform-benign}. We sample models from different families that cover Convolutional Neural Networks (CNNs) and Vision Transformer (ViT): \{VGG-19-BN~\cite{simonyan2014very}, ResNet-50~\cite{he2016deep}, DenseNet-121~\cite{huang2017densely}, InceptionV3~\cite{szegedy2016rethinking}, MobileNet-v2~\cite{sandler2018mobilenetv2}, ViT-L-16, ViT-L-32~\cite{dosovitskiy2020image}, Swin-T~\cite{liu2021swin}\}. We use $1000$ ImageNet-like RGB images from the NeurIPS17' challenge~\cite{neurips17challenge}. The dataset has $1000$ classes same as ImageNet and all images in the size of $224\times224$.


\noindent\textbf{Attack settings.} We focus on targeted attacks, as they are more challenging than untargeted ones and align with our transform-dependent attack formulation. For simplicity, we consider $N=3$ transform parameters $\{\bar{\theta_i}\}_{i=1}^3$, though in principle, $N$ can be extended to larger numbers. The goal is to deceive the model into providing three distinct, desired target labels when the victim model is provided with the corresponding transformed perturbed images. We randomly select three unique targets $\{y^\star_i\}_{i=1}^3$ from ImageNet classes, ensuring that they differ from the ground-truth label. For optimization, we used $500$ iterations for PGD with a step size of $\alpha=5\times 10^{-4}$ for sufficient convergence.
% \Salnote{Changed a bit. Make sure this is correct?} \ytan{Re: correct}
%
% We use $\ell_\infty$ norm bound, with visually imperceptible perturbation budget $\|\delta\|_\infty \leq 10$ for experiments presented in~\cref{subsec:whitebox}.

% \input{tables/tab-cls-asr}
 
\noindent\textbf{Evaluation metrics.} 
We evaluate the transform-dependent attack performance using the Attack Success Rate (ASR). Specifically, for a perturbed image transformed as $T(\mathbf{x}+\delta;\theta_i)$, we check whether the network prediction matches target label $y^*_i$. We report ASR for each transform parameter $\bar{\theta_i}$ over $N_r(\bar \theta_i)$, where $N_r(\bar \theta_i)$ includes series of $\theta$ samplings iterated with a small step-size (detailed in \cref{subsec:whitebox}), and report ASR averages over all samplings within $N_r(\bar \theta_i)$.

\subsection{Transform-dependent attacks on classifiers}
\label{subsec:whitebox}
We present transform-dependent attacks using different image transforms with prevalent applications in real world scenarios, including geometric transforms (e.g., scaling, blurring), photometric transforms (e.g., Gamma correction) and image compression (e.g., JPEG).
%
For each transformation, we selected the transformation parameters $\{\theta\}$ in the range that has minimum impact on the model accuracy without perturbation. 
%
We then evaluate ASR (\%) on transform-dependent adversarial examples.
%
For reference, we provide classification accuracy evaluation on clean images under same transforms in the supplementary (see \cref{tab:cls-acc}).





% \subsubsection{Attacks for fixed transforms}
% %
% In this section, we will explain the attacks for discrete values of transform parameters. \cref{tab:cls-asr} summarizes the ASR for the transform-dependent attacks with three target labels assigned to three discrete values of transform parameters. In the next section, we expand the attacks over a range of transform parameters. 

% \noindent\textbf{Scale-dependent attacks.} 
% In real-world applications, images can be presented and displayed at different scales and resolution. To mimic this effect, we employ scaling transformation and create targeted attacks according to the image scale/resolution. For the scale-dependent attacks, we selected the scaling factor $S\in\{0.5, 1.0, 1.5\}$. We used bilinear interpolation to apply the corresponding scaling transforms that result in transformed images with $112\times112$, $224\times224$, and $336\times336$ pixels.
% %

% \noindent\textbf{Blur-dependent attacks.} 
% We employ Gaussian blur to create blur-dependent attacks, mimicking images captured out-of-focus in the real world.
% We fix the Gaussian kernel size to $5$ and vary standard deviation $\sigma$ as the transform parameter. Specifically, we choose $\sigma\in\{0.5, 1.5, 3.0\}$ for creating small, mid, and severe levels of blurry effects.
% %


% \noindent\textbf{Gamma-dependent attacks.} 
% Beyond linear transformations, we also consider gamma correction---a widely used technique for compensating the non-linear characteristics of display devices, also generally used for simulating lighting condition variation in deep networks  training.  We adopt $\gamma \in \{0.5, 1.0, 2.0\}$ to simulate bright, normal, and dark lighting conditions. The visual effects can be seen in the second row of~\cref{fig:intro}.


% \noindent\textbf{Compression-dependent attacks.} 
% We demonstrate that images compressed at different levels exhibit varying attack effects. Specifically, we consider widely used JPEG and implement differentiable JPEG compression, following the method in \cite{shin2017jpeg}. For the JPEG transform, we use compression qualities $Q\in\{20, 50, 80\}$ as the transform parameters. The higher value of $Q$ indicates less compression loss.

% We present the ASR of achieving transform-dependent attacks with three target labels on different whitebox models in \cref{tab:cls-asr}. 
% %
% The results demonstrate that our method provides successful transform-dependent targeted attacks in all the settings across all the models. This amounts to three distinct target labels for the same (perturbed) image and same transform but three different transform parameters. 
% % \Salnote{1-2 lines to explain key takeaway from the table?? Is the ASR nearly 100\% in all the cases. If not, why not???} 
% From the table, we observe that different models exhibit varying levels of adversarial vulnerability to transform-dependent attacks. Transform-dependent attacks achieve above $90\%$ ASR on most convolutional networks and $78.97-89.87\%$ ASR on InceptionV3, depending on the transform function used. For ViT-based models, the ASR varies from $68.77\%$ to $93.67\%$ depending on the transform function and the image patch size. % Among the four  transform functions we used in our experiments, scaling and gamma transforms provide high ASRs on almost all the models. 

% % Results in~\cref{tab:cls-asr} show that our attack can successfully provide three distinct transform-dependent labels for the same (perturbed) image. 

% % Results in the scale-dependent attack part of ~\cref{tab:cls-asr} show that perturbed images effectively provides the desired target labels for the corresponding scaling factors. 

% % Results in~\cref{tab:cls-asr} show that three different blur levels achieve high success rate for the corresponding targeted attacks on all the models. 

% % Results in~\cref{tab:cls-asr} demonstrate that our method provides successful transform-dependent attacks with this non-linear image transformation, which amounts to three distinct target labels for the same (perturbed) image under three different lighting conditions.





% \subsubsection{Consistent attacks for a transform range} \label{subsec:whitebox-range}
% In this section, we discuss the experiments for generating consistent targeted attacks over a range of transform parameters. 
\cref{tab:cls-asr-range} summarizes the ASR for the transform-dependent attacks with three target labels assigned to three distinct ranges of the transform parameters. 
%
We generate these attacks using the method described in \cref{eq:attack-transform-dep-range}. We further demonstrate that the attacks generated in this manner maintain transform-dependent properties with small parameter variations. In \cref{sec:transfer}, we demonstrate that such attacks are also transferable to blackbox models.

% \noindent\textbf{Whitebox attack results.} 
We follow the same experiment settings as described above, but define the transform parameters over a range of scaling, blur, gamma, and compression ($S$, $\sigma$, $\gamma$, and $Q$). 
In particular, we select a neighborhood with interval radius $r=0.1$ for scaling, blurring, gamma correction, and $r=1$ for JPEG compression. The resulting parameter ranges are as follows: scaling $S \sim \{[0.4,0.6], [0.9,1.1], [1.4,1.6]\}$, blurring $\sigma \sim \{[0.4,0.6], [1.4,1.6], [2.9,3.1]\}$, gamma correction $\gamma \sim \{[0.4,0.6], [0.9,1.1], [1.9,2.1]\}$, and JPEG compression $Q \sim \{[19,21], [49,51], [79,81]\}$. 

We present the ASR of achieving consistent transform-dependent attacks on different whitebox models in \cref{tab:cls-asr-range}. 
% Compared to \cref{tab:cls-asr}, the ASRs over a range of transform parameters exhibit minor drops because enforcing targets for more transform parameters increases the difficulty of solving the optimization problem, but they remain close to the values obtained with discrete parameters (\cref{tab:cls-asr}). The key advantage of generating consistent attacks for a range of transform parameters is that they remain effective with small modifications in $\theta$. 
%
% \Salnote{Anything else that is special in the table to highlight???} \ytan{Re: updated.}

% \input{figures/vis-cls}

% \subsubsection{Loss landscape of transform-dependent attacks} 
%
\noindent\textbf{Loss landscape of transform-dependent attacks.} The loss landscape of the surrogate models can help us evaluate the sensitivity of the attacks over the transform parameters. In this vein, we evaluate the loss function~\cref{eq:attack} corresponding to three target labels with different attacks and transform parameters. In \cref{fig:loss}, we present the loss landscape for ResNet50 model as we apply different transforms over a range of transform parameters to the adversarial examples generated in \cref{tab:cls-asr} and \cref{tab:cls-asr-range}. Different colors in \cref{fig:loss} correspond to different target labels; solid lines correspond to average loss and shaded area corresponds to the standard deviation of loss over the entire experimental dataset. 
%
Top row corresponds to \cref{tab:cls-asr}, where one perturbation is generated to provide three target labels for three distinct values of transform parameters. Bottom row corresponds to \cref{tab:cls-asr-range}, where one perturbation is generated to provide three target labels for three distinct ranges of transform parameters. 

We observe in \cref{fig:loss} that the minimum loss values occurs at the desired transform parameter values/ranges across all four transformations. This indicates that adversarial examples successfully learned to embed targeted attacks that are triggered when a desired transformation is applied.
%
We also observe that different transform-dependent adversarial examples have varying levels of sensitivity to the transform parameters. In the top row, where perturbations are generated for three discrete transform parameters, scaling and JPEG compression are more sensitive to the transform parameters, whereas blurring and gamma correction are less sensitive. In bottom row, where perturbations are generated for three ranges of transform parameters, all four transformation are able to achieve attack success within a range of parameters. In the next section, we discuss how the perturbations generated for a range of transforms also provide better transfer attacks for blackbox models. 

% Figures in the first row are computed over the surrogate model, w
% %
% For reference, the second row shows the loss landscape of adversaries \ytan{todo update} \cref{subsec:whitebox-range} being forwarded to a non-surrogate model, we observe that loss curves for different targets do not exhibit a transform-dependent pattern and present a similar trend.




% \subsubsection{Visual examples} 
% In~\cref{fig:cls}, we provide examples of each image transformation we experimented with in~\cref{subsec:whitebox}. The examples show that our attacks can trigger various targeted attacks under a variety of image transformations while maintaining good imperceptibility in terms of human visual and network level --- clean images under the same condition network provide correct predictions. This demonstrates the decent controllability and stealthiness introduced by our attack formulation.

% \Salnote{Do we have examples for range of transforms or do we want to modify this figure to add captions for range of transforms? }


\input{tables/tab-cls-bb}

\subsection{Attacks against blackbox and defended models} \label{sec:transfer}
%
One advantage of transform-dependent attacks is that the generated adversarial perturbations become a function of the transform parameters. We exploit this property to attack for different blackbox models. 
%
Since we can only access the outputs of the blackbox models for different inputs, we query the models with different transformed versions of the perturbed images $T(x+\delta; \theta)$ on blackbox models for a range of $\theta$. 
%
We evaluate the transfer success rate of such attacks on blackbox models using a maximum of $3$ queries. 

For any given image $x$ with the perturbation $\delta$ generated for a surrogate model, we sample the transform parameters $\theta$ within the parameter neighborhoods used for adversarial examples training in \cref{tab:cls-asr-range} (i.e., $\theta \sim N_r(\bar\theta)$). We seek a transformed adversarial example $T(x+\delta; \theta)$ as a function of $\theta$ that successfully deceives the blackbox model to provide the desired transform-dependent target labels. We can describe the attack process for a blackbox model $f_\text{bb}$ as 
\begin{equation}\label{eq:attack-transform-dep-bb}
    \text{find } \theta_i^* ~~~ \text{s.t.}~~~f_{\text{bb}}(T(x+\delta;\theta_i^\star)) = y_i^\star;~  \theta_i^\star \in N_r(\bar \theta_i).
\end{equation}
%
Note that $\delta$ represents the perturbation generated for a surrogate model (e.g., ResNet50) for the desired target labels at the corresponding transform parameter ranges, as described earlier. {When attacking the $f_{\text{bb}}$, we uniformly search within the $N_r(\bar \theta_i)$ corresponding to the target $y_i^\star$ with the sampling size $0.1$ resulting $3$ queries for each transform parameter $\theta_i$ (e.g., search space is $\{0.4,0.5,0.6\}$ for scaling at $\bar \theta_i=0.5$).} An attack is considered successful if we can find an adversarial example that deceives the blackbox model into predicting the desired target label (as described in~\cref{eq:attack-transform-dep-bb}). 
% \Salnote{Report specific process and max number of queries somewhere here..? For example, we sweep over $\theta_i$ using binary search with at most xx queries per attack?}

% \Salnote{Do we need untargeted attacks here or move to supplementary?}
%
We report the results for transfer attack success rate of our method and its comparison with other methods in \cref{tab:attack-transfer-bb}. 
%
In addition to the targeted attacks demonstrated in previous sections, we also include the untargeted attack success rate in \cref{tab:attack-transfer-bb}. This is because most of the recent transfer attack methods mainly focus on untargeted attacks, which consider attack successful as long as the blackbox model fails to provide the correct label (i.e., $f_{\text{bb}}(T(x+\delta;\theta_i^\star) )\neq y_i$).
% For a fair and comprehensive comparison with these methods, we used $\varepsilon=8$ and introduced the model MobileNet-v2~\cite{sandler2018mobilenetv2} in this experiment. We provide the evaluation of the blackbox transfer attack success of our method in both untargeted and targeted settings in \cref{tab:attack-transfer-bb}.
%
% \Salnote{I do not understand the mention of MobileNetv2 here. Why do we need to point it out. Did we point out other whitebox models elsewhere???} \ytan{Removed and added MobileNetv2 to table 1 and 2 like other whitebox models.}

Our method achieves untargeted/targeted ASRs comparable to recent transfer-based methods \cite{xiaosen2023rethinking,wei2023enhancing,li2024improving} without any special adaptation but data augmentation over the range of parameters.
%
Note that most of the existing transfer-based methods report impressive results only for untargeted attacks. The transfer ASR for targeted attacks remains quite low with a small perturbation budget (e.g., $\varepsilon=8$). For reference, we include results from BPA~\cite{xiaosen2023rethinking}, SU~\cite{wei2023enhancing} and ILPD~\cite{li2024improving} with the same setup (e.g.,  dataset, perturbation budgets), surrogate model (ResNet50), and target labels. 

% \Salnote{Need to add a few more closing lines to this section. What is the significance of the table? Query budget, when is transfer successful, when is it challenging etc...}

The results in \cref{tab:attack-transfer-bb} demonstrate that scale- and blur-dependent attacks achieve remarkable success for untargeted and targeted attacks. Note that while all the listed methods attack blackbox models for a single attack with a single perturbation, our attacks demonstrate that one perturbation is capable of achieving multiple targeted attacks on blackbox models. This is a more challenging task and has been demonstrated for the first time. Among the transforms, scale-dependent attacks are slightly more transferable than blur-dependent attacks. For targeted attacks, success mostly occurs at larger scaling factors, while for untargeted attacks, it mostly occurs at smaller scaling factors. These results show that by leveraging the image transform space in adversarial example generation, with negligible search cost at test time, attacks can be made more transferable to blackbox models, demonstrating the effectiveness of our attack formulation in a challenging practical setup.




% \noindent\textbf{Attacks over the range of transform parameter.}
% \ytan{We also evaluate adversarial examples within specific intervals to see whether transform-dependent perturbations can misclassify images into the desired target labels over a range of transform parameters beyond fixed values evaluated in~\cref{tab:cls-asr}.}

\input{tables/tab-cls-rob}

% \subsection{Attacks against robust models and defenses}
% \label{subsec:robust}
\noindent\textbf{Attacks against defended models}
To further evaluate the effectiveness of the transform-dependent attacks, we assess their performance on five defense methods: robust models with adversarial training (AT)~\cite{goodfellow2014explaining}, HGD~\cite{liao2018defense}, Randomized Smoothing (RS)~\cite{cohen2019certified}, JPEG compression (JPEG)~\cite{guo2017countering} and NPR~\cite{naseer2020self}.


% \noindent \textbf{Attacks against robust models.} 
We employ ResNet50 models adversarially trained on the ImageNet dataset from~\cite{robustness}. Specifically, we select pre-trained models robustly against $\ell_\infty\leq4,8$ untargeted attack adversaries. These models have lower accuracy than normally trained models~\cite{shafahi2019adversarial} but they are robust in the way that they can provide consistent predictions for perturbed images to the clean images; that is, model consistency defined as $f(\mathbf{x}+\delta)=f(\mathbf{x})$. 
% \Salnote{WHAT THE HECK IS $x^\star$ here???}\ytan{updated all $x^\star$ to consistent notation: $\mathbf{x}+\delta$}

% \Salnote{WHAT IS THE TOPIC SENTENCE HERE??? It is certainly not the fairness of evaluation and perturbation budget!!!}
%
{Evaluating the transform-dependent attacks on robust models trained with different $\ell_\infty$-norm bounded adversarial perturbations requires carefully designed attack plans and ensuring fairness in testing conditions.} We used the same perturbation budget as the model adversarial training settings. For instance, we used $\varepsilon=4,8$ for attacking ResNet50-eps4,8, respectively, in \cref{tab:attack-rob}. We formulate attack plans to disrupt the model predictions, (i.e., lowering model consistency), and use an ASR metric that is similar to untargeted ASR. In particular, if the model fails to provide consistent predictions for images with and without transformations, then the attacks are considered successful (i.e., $f(T(\mathbf{x}+\delta;\theta)) \neq f(\mathbf{x}+\delta)$). We formulate the attack plan using transform parameters $S\in\{0.5, 1.5\}$, $\sigma\in\{0.5, 1.5\}$, $\gamma\in\{0.5, 2.0\}$ and $Q\in\{50, 100\}$ with $2$ randomly select targets from the label space. 
% \Salnote{Why do we have 2 transform-dependent attack labels here, whereas the rest of the paper has 3 attack labels???}

Results in~\cref{tab:attack-rob} show that our attacks effectively disrupt the robust models in the transformation space. The prediction consistency of robust models are not affected by the perturbation (i.e., $f(\mathbf{x}+\delta)=f(\mathbf{x})$) for images under the original condition (e.g., when $S=1.0$, $\gamma=1.0$, $Q=100$ and no blurring). The models fail to provide consistent predictions as the perturbed images undergo different transformations (i.e., $f(T(\mathbf{x}+\delta;\theta))\neq f(\mathbf{x}+\delta)$). For reference, we provide model consistency evaluation of experimental models on transformed clean images $f(T(\mathbf{x};\theta))=f(\mathbf{x})$ in the supplementary \cref{tab:attack-rob-acc}. 
% \Salnote{Where in supplementary?}

\noindent \textbf{Evaluations on other defense methods.} 
We also evaluate the performance of our attacks under the untargeted setting against four defenses applied to the surrogate model ResNet50, following the settings in one of the recent transfer attacks BPA~\cite{xiaosen2023rethinking}. We use the ground-truth label ($y$) as the target in \cref{eq:attack-transform-dep} for all transform parameters $\theta_i$ and maximize the loss as untargeted attacks in our attack optimization. In \cref{tab:attack-defense}, we report the untargeted ASRs averaged over all the transform parameters. For a fair comparison with BPA methods, we used $\varepsilon=8$ in these experiments, and our attack archives overall better performance than BPA on the same benchmark. These results suggest that transform-dependent attacks can bypass existing defense methods by leveraging the transformation space beyond adversarial-robust models evaluated in \cref{tab:attack-rob}. 


\input{tables/tab-cls-defense}


% \input{tables/tab-cls-defense}
% \input{tables/tab-cls-bb}



% \subsection{Transfer attacks against blackbox models}
% \label{subsec:transfer}
% In this section, we evaluate the transfer success rate of our attacks on blackbox models.  

% Instead of generating attacks for a fixed scaling factor $S$ and blurring $\sigma$ as in \cref{subsec:whitebox} (i.e., $S=\{0.5, 1.0, 1.5\}$ and $\sigma=\{0.5, 1.5, 3.0\}$), in this experiment we generate attacks over a range of parameters $S$ and $\sigma$ (i.e., $S \sim \{[0.4,0.6], [0.9,1.1], [1.4,1.6]\}$ and $\sigma \sim \{[0.4,0.6], [1.4,1.6], [2.9,3.1]\}$), 
% which can contribute to transfer attack success according to~\cite{athalye2018synthesizing}.

% We provide the evaluation of blackbox transfer of our attacks in untargeted and targeted settings in \cref{tab:attack-transfer-bb}.

% \ytan{TODO: make experiment complete, add results for other two transformations in the TPAMI version}

% Our method achieves untargeted/targeted ASRs comparable to recent transfer-based methods ~\cite{xiaosen2023rethinking,wei2023enhancing,li2024improving} without any special adaptation.

% Note that most of the existing transfer-based methods report impressive results only for untargeted attacks. The transfer ASR for targeted attacks remains quite low in a small perturbation budget. For reference, we include results from BPA~\cite{xiaosen2023rethinking}, ILPD~\cite{li2024improving} and SU~\cite{wei2023enhancing} with the same dataset, surrogate models (ResNet50), and target labels. 
 
% For a fair and comprehensive comparison with these methods, we used $\varepsilon=8$ and introduced the model MobileNet-v2~\cite{sandler2018mobilenetv2} in these experiments.

\input{figures/vis-det-enhance}

\subsection{Extension to object detection task}
\noindent \textbf{Models and dataset.} 
For the object detection task, we utilize detector models pretrained on COCO 2017 dataset~\cite{lin2014microsoft} from \texttt{MMDetection}~\cite{mmdetection}. Specifically, we select two one-stage models \{YOLOv3~\cite{redmon2018yolov3}, FCOS~\cite{tian2019fcos}\}, two two-stage models \{Faster R-CNN~\cite{ren2015faster}, Grid R-CNN~\cite{lu2019grid}\} and one ViT-based model DETR~\cite{carion2020end}. For dataset, we use 500 images from COCO 2017 validation that contain objects in $3$ unique categories denoted as $A, B \text{ and } C$. 

\input{tables/tab-det}

\noindent \textbf{Attack scenario and evaluation.} 
We consider scaling transformation out of the simplicity and consistency with previous experiments and continue with the same scaling factors $S\in\{0.5, 1.0, 1.5\}$ and try to achieve attack effects namely scale selective hiding. Our objective is to conceal objects belonging to one of the categories from $A$, $B$, and $C$ in the detection results of $T(\mathbf{x};0.5), T(\mathbf{x};1.0) \text{ and } T(\mathbf{x};1.5)$, i.e., hide all $A$ objects when image scaling to $0.5\times$, hide all $B$s when scaling to $1.0\times$ and hide all $C$s when scaling to $1.5\times$.

In this scenario, we measure ASR as \textit{the ratio of successfully hidden objects in the final detection result} of the corresponding scaled input image.


\noindent \textbf{Results and visual examples.} 
\cref{tab:attack-detector} show that over most R-CNN-based detectors, the scale-dependent attack effects are successfully triggered when adversaries scale to the corresponding image size. In~\cref{fig:det}, we provide a successful example of selective hiding effects and utilize the GradCAM~\cite{selvaraju2017grad} to visualize the feature level understanding of the detector. Our results show that transform-dependent attacks can be extended to more complex dense prediction models.


\input{figures/vis-det}




==> archive/intro.tex <==
\section{Introduction}
\label{sec:intro}
% \IEEEPARstart{A}{dversarial}
Adversarial attacks on deep neural networks have traditionally been studied through the lens of  imperceptible perturbations that can fool models into misclassifying inputs~\cite{goodfellow2014explaining,kurakin2016adversarial, madry2017towards,dong2018boosting,zou2020improving,wang2021admix,wang2023structure,xie2019improving,dong2019evading, lin2019nesterov}. In many real cases, inputs can undergo different transformations due to changes in viewpoint, lighting conditions, and resolution with little to no perceptual change. Prior work has attempted to make adversarial attacks robust to such input transformations by optimizing over the expectation of the attack objective under a distribution of transformations. For instance,  the expectation over transformation (EOT) framework \cite{athalye2018synthesizing} seeks transforma-invariant (or -independent) attacks that robust to variation of input transformations.

\input{figures/fig-intro-v2}
\input{figures/fig-intro}

In this work, we explore an entirely new dimension of adversarial attacks --- transform-dependent adversarial attacks. Unlike conventional approaches that aim for invariance to transformations, we uncover a new threat: a single, carefully crafted perturbation can induce a wide range of targeted mispredictions, controlled by the applied transforms. This transform-dependent effect not only enhances stealthiness, extending beyond visually imperceptible noise, but also introduces a potential defense mechanism --- preventing sensitive information disclosure when image enhancement transforms risk exposing private content, as demonstrated in \cref{fig:intro2}.
%
% Imagine a seemingly benign image that turns into an adversarial example with different target labels when resized, rotated, or compressed with different parameters. 
%
% This redefines what it means for an input to be adversarial--the adversarial nature is not simply an intrinsic property, but a complex capability induced by the perturbation to react differently under different transformations. 
%
% Figure~\ref{fig:intro}
\cref{fig:intro} presents examples of transform-dependent adversarial attacks, showing how a single perturbation can lead to different target labels depending on the transformation applied. Stealthiness is achieved by optimizing attack effects to remain latent under normal conditions, only being triggered when transformation parameters deviate from the original image state.


Our analysis of this new class of controlled, transform-dependent adversarial attacks reveals a profound threat for which current defenses are ill-prepared due to the expanded adversarial space introduced by image transforms. Our results highlight the significant vulnerability of modern deep learning models to these attacks. We demonstrate that a single additive perturbation can encode a remarkable diversity of targeted adversarial effects, each triggered by predefined input transformations. Unlike conventional attacks, which rely on isolated and static perturbations with fixed post-training effects, our approach introduces dynamic, controllable threats—capable of manifesting in drastically different ways depending on how the input is transformed.


\noindent We summarize our main contributions as follows.
\squishlist
\item We introduce the novel concept of transform-dependent adversarial attacks, where a single additive perturbation can embed multiple targeted mispredictions that are triggered by predefined transforms on the input image.
%
\item We showcase the versatility and practicality of proposed attacks through extensive experiments across models, tasks, and transforms, demonstrating how a single perturbation yields diverse, controllable adversarial effects.
%
\item Our study on defended and blackbox models suggests that transform-dependent attacks can achieve high blackbox transfer success rates and bypass existing defenses (e.g., adversarial training, randomized smoothing). 
%
% \item Our experiments highlight different factors that influence the effectiveness of such controllable perturbations (e.g., the choice of transform functions and model architecture).
%
\item We demonstrate the real-world implications of transform-dependent perturbations as a defense by extending our results to object detection, enabling selective object hiding based on image enhancement transforms.
%
\squishend

Our attack formulation represents the initial endeavor to integrate multiple attack effects in a single adversarial perturbation, which can be dynamically activated in coordination with image transforms, enabling attacks deployment controllable.
%
Our work questions the fundamental assumption in adversarial machine learning --- that an input example is either benign or adversarial. Our work forces a conceptual paradigm shift, as adversarial perturbations can now encode metamorphic properties that reveal different attack effects based on transformations applied to the input. Defenses can no longer simply aim to detect static perturbations, but must grapple with the chameleon-like nature of our transform-dependent adversarial attacks. 

==> archive/method.tex <==
\section{Method}
\label{sec:method}


\subsection{Preliminaries}
We consider additive perturbations for adversarial attacks~\cite{szegedy2013intriguing,goodfellow2014explaining,madry2017towards} that generate an adversarial example as $\mathbf{x}+\delta$, where $\delta$ is an adversarial perturbation for a given image $\mathbf{x}$. Given a well-trained model $f$ that provides correct prediction, $f(\mathbf{x})=y$. We can learn $\delta$ for an untargeted adversarial attack  such that $f(\mathbf{x}+\delta) \neq y$ (i.e., the  prediction does not match the correct label) or a targeted attack such that $f(\mathbf{x}+\delta) = y^\star$  (i.e., the prediction is the desired target label $y^\star$). To keep the perturbation imperceptible, $\delta$ is usually bounded within the $\ell_p$ norm ball $\|\delta\|_p \leq \varepsilon$. In general, targeted adversarial attacks can be generated by solving the following optimization problem:
\begin{equation}\label{eq:attack}
    \min_{\delta}~\mathcal{L}(f(\mathbf{x}+\delta), y^\star)\quad \text{s.t. } \|\delta\|_p \leq \varepsilon.
\end{equation}

% 
A general choice for the loss function $\mathcal{L}$ is the training loss for the corresponding tasks. Several algorithms have been proposed to solve this optimization problem; notable examples include  FGSM~\cite{goodfellow2014explaining}, PGD~\cite{madry2017towards}, MIM~\cite{dong2018boosting} and Auto-Attack~\cite{croce2020reliable, croce2021mind}. In this work, we focus on PGD attacks for their simplicity and effectiveness. PGD iteratively solves the attack optimization problem as 
\begin{equation}\label{eq:PGD}
    \delta^{t+1} = \Pi_{\varepsilon} \left( \delta^{t} - \alpha~ \mathbf{sign} (\nabla_{\delta}\mathcal{L}(f(\mathbf{x}+\delta^{t}), y^\star)) \right),
\end{equation}
where $\delta^t$ denotes perturbation at iteration $t$ that is updated using sign of gradient with step size $\alpha$. $\Pi_{\varepsilon}$ denotes an operator that projects the updated $\delta^t$ back to the $\ell_p$-norm ball and obtain $\delta^{t+1}$.


\subsection{Transform-dependent attacks}
Let us define the image transform function as $T(\mathbf{x};\theta)$ that transforms the input image $\mathbf{x}$  according to the given transform parameter $\theta \in \Theta$. Applying the transform function over clean input images does not cause significant degradation in the accuracy of networks that are properly trained with data augmentation techniques~\cite{rowley1998rotation,jaderberg2015spatial, marcos2017rotation}. In other words, the output of the transformed images remains same as the original image:   
\begin{equation}\label{eq:transform-benign}
    f(T(\mathbf{x}; \theta)) \sim y.
\end{equation}

To introduce image transform-dependent effects in adversarial examples, we incorporate the transform function in the attack generation. Specifically, we aim for transform-dependent targeted attacks with target label $y^\star_i$ for the corresponding transform parameter $\theta_i$.  


%
In the most general form, we assume $\boldsymbol  \theta$ and $\mathbf{y}^\star$ represent two vectors with $N$ discrete targets embedded in the transform-dependent attacks as $\boldsymbol\theta = \{\theta_i\}_{i=1}^N$, $\mathbf{y}^\star = \{y^\star_i\}_{i=1}^N$. 
%
The attacker can select a mapping for \textbf{parameter-target pairs} that trigger the label $y_i^\star$ for a given transform parameter $\theta_i$, or choose the $y_i^\star$ as true label $y_i$ for certain transform parameters where the adversarial examples are intended to act as ``benign'', for better stealthiness. 
%
% The transform parameter can either be assigned a single predefined value or sampled randomly from a predefined range.
%
We seek to generate a single transform-dependent perturbation $\delta$ as a solution of the following optimization problem:
\begin{equation}\label{eq:attack-transform-dep}
    \min_\delta~\sum_i \mathcal{L}(f(T(\mathbf{x}+\delta; \theta_i)), y^\star_{i}) \quad {\text{s.t. }\|\delta\|_p \leq \varepsilon}. 
\end{equation}
%
At the test time, the perturbed image can be created as $\mathbf{x} + \delta$, the transform-dependent adversarial examples can be created as $T(\mathbf{x} + \delta;\theta_i)$, and attacks can be triggered by providing malicious $\theta_i$, resulting in transform-dependent effects.


To enhance the robustness of the transform-dependent attacks against small variation on transform paramters, we employ the idea from EOT \cite{athalye2018synthesizing}, optimize perturbations that are continues to provide desired attacks with small changes in the transform parameters. 
%
To achieve this goal, we incorporate expectation over transforms data augmentation~\cite{athalye2018synthesizing} in the optimization problem. 
Specifically, we search for the perturbation $\delta$ that provides desired target label $y^\star_i$ over a range of transform parameters $\theta_i$ around the neighborhood of $\bar \theta_i$ by solving the following optimization problem: 
%
\begin{equation}\label{eq:attack-transform-dep-range}
    \min_\delta~\underset{\theta_i \sim N_r(\bar \theta_i)}{\mathbb{E}}~\sum_i \mathcal{L}(f(T(\mathbf{x}+\delta; \theta_i)), y^\star_{i}) \quad {\text{s.t. }\|\delta\|_p \leq \varepsilon}, 
\end{equation}
where $N_r(\bar \theta) = \{ \theta \in \Theta \mid  \left\| \theta - \bar \theta \right\| < r \}$ represents a uniform distribution around mean $\bar \theta$ with interval radius $r$. The generated perturbation can provide consistent attacks over a range of parameter values instead of discrete values.

We also observe that the perturbations generated for a range of transforms and parameters (with data augmentation) can provide successful transfer attacks for the blackbox models, consistent with findings in \cite{lin2019nesterov, transfer attacks}. We provide additional details in \cref{sec:transfer}, where perturbations generated for a single surrogate model can fool multiple blackbox models with different architectures. Furthermore, the blackbox transfer attacks maintain transform-dependent attack properties as the blackbox models predict the desired transform-dependent target labels when provided with transformed versions of the input images.

\subsection{Transform functions}
We primarily focused on transform functions with two properties. The first desired property for generating adversarial attacks is the differentiability of the selected transforms $T(\mathbf{x}; \theta)$ so that it can be used with gradient-based attack algorithms and the gradient of loss function with respect to $\delta$ can be written as 
$
    \nabla_{\delta}\mathcal{L}(f(T(\mathbf{x}+\delta; \theta)), y^\star) = 
    \frac{\partial \mathcal{L}}{\partial f}
    \frac{\partial f}{\partial T}
    \frac{\partial T}{\partial \delta}. 
$
The second key property is controllability so that the transform-dependent attack can be controlled by $\theta$. The attacker can customize transform-dependent effects by controlling $\theta$ for the transform function.

Based on these two properties, we adopt a wide range of image transform techniques as transform functions, covering spatial, photometric transforms, and image compression.
While we focus our discussion on scaling, blurring, and gamma correction that are mainly used in the experiment, attack principles can be extended to many other image transforms that follow the above properties.
%
For scaling, transform parameter is the scaling factor $S$; $T$ transform image $\mathbf{x} \in \mathbb{R}^{H\times W\times3}$ into $T(\mathbf{x};\theta=S) \in \mathbb{R}^{S H\times S W\times3}$. Commonly used scaling methods like bilinear and bicubic interpolations are differentiable operations.
For blurring, typically Gaussian blur, the transform parameter is the standard deviation $\sigma$ used to create the Gaussian kernel and the transformed image can be represented as $T(\textbf{x};\theta=\sigma)$.
For Gamma correction, transformed image can be represented as $T(\mathbf{x};\theta=\gamma) = A \mathbf{x}^{\gamma}$, where $\gamma$ is the transform parameter and $A$ is a normalizing constant. 
While JPEG compression is non-differentiable due to quantization process, we can also use that for transform-dependent attacks. For this purpose, we leverage a differentiable approximation $JPEG_{\text{diff}}$ from \cite{shin2017jpeg} and the JPEG-transformed image can be represented as $T(\textbf{x};\theta=Q) = JPEG_{\text{diff}}(\textbf{x},Q)$, where $Q$ is the compression quality.


==> archive/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Adversarial attacks and defenses}
Adversarial attacks were initially introduced as visually imperceptible perturbations \cite{goodfellow2014explaining}, capable of causing false predictions in untargeted attacks or inducing specific misclassifications in targeted attacks \cite{}. Adversarial vulnerabilities have been found across various deep learning architectures and tasks, including classification and object detection \cite{CNN, Transformer, classifiers, obj det}. However, in the conventional paradigm, a single post-training perturbation can achieve only one fixed attack outcome, offering limited control over adversarial effects. Likewise, existing defenses operate under the assumption that an input is either benign or adversarial, without considering dynamic adversarial behaviors \cite{cite some adv defense}. 
%
In this work, we challenge this paradigm by leveraging image transforms in adversarial optimization. Our proposed transform-dependent attacks introduce a new level of controllability, allowing a single perturbation to induce multiple, transform-driven attack effects. This approach not only expands the adversarial threat landscape but also effectively bypasses several widely used defenses.

% \subsection{Known properties of adversarial examples}
% Adversarial examples possess several intriguing properties that have been extensively studied in the literature. Besides imperceptibility, researchers have explored and imposed several other properties, such as transferability, universality, and transformation robustness. An intriguing property of adversarial examples is their transferability across different models \cite{papernot2017practical, tramer2017ensemble,xiaosen2023rethinking,wei2023enhancing,li2024improving}. Adversarial examples generated for one model can often fool other models trained on the same task, even if they have different architectures or were trained on different datasets. To enhance transferability, ensemble-based and momentum-based attacks are proposed. Researchers have also discovered the existence of universal adversarial perturbations (UAPs) \cite{moosavi2017universal}, which are single noise patterns that can cause mis-classification across a wide range of input samples, rather than being tailored to individual samples. While UAPs underscore the potential for broad applicability of a single perturbation, they do not inherently address dynamic control over the prediction outcomes based on input transformations. A foundational area of relevance is the body of work centered on the robustness of machine learning models against input transformations. Expectation Over Transformation (EOT) provides a framework for generating adversarial examples that remain effective under a range of transformations, such as rotation and scaling \cite{athalye2018synthesizing}. This methodology enables physical attacks by considering the variability of real-world inputs in crafting adversarial attacks. These studies collectively highlight the evolving understanding of adversarial perturbations, however they are focusing on singular attacks and do not provide insights on dynamically controllable perturbations which we specifically investigate in this paper.


% \subsection{Differentiable image transformations}
% The core premise of transform-dependent attacks relies on applying differentiable transformations to input images during the adversarial optimization process. A wide range of image transformations have been adapted to differentiable forms, enabling their seamless integration into gradient-based optimization frameworks. Geometric transformations like scaling, translation, and rotation are differentiable thanks to the availability of interpolation techniques like bilinear and bicubic interpolation, which can be expressed as differentiable operations \cite{jaderberg2015spatial}. Photometric transformations such as gamma correction, brightness/contrast adjustments, and color space augmentations can be made differentiable by formulating them as pointwise operations on the input tensor. Gaussian blurring, which is non-differentiable due to the discrete nature of the kernel, can be approximated using isotropic kernels expressed as a linear combination of Gaussian basis functions, enabling differentiation. Even low-level operations like JPEG compression, which involves quantization, can be approximated using differentiable formulations that model the quantization effects \cite{shin2017jpeg}. The choice of transformations is motivated by their prevalence in real-world imaging conditions and data augmentation pipelines. By composing a diverse set of spatial, photometric, and signal transformations, we can optimize for adversarial perturbations that exhibit controllable behavior under a wide range of input corruptions that may occur during deployment.


\subsection{Image transformation in adversarial attacks}
In adversarial attack literature, image transforms have primarily been leveraged for two purposes: 
1) Generating transform-invariant adversarial examples that remain effective under input corruptions \cite{athalye2018synthesizing,kurakin2018adversarial,Lennon_2021_ICCV}, and transferable adversarial examples that remain adversarial across models that are differ from the model used in the attacks generation process \cite{zou2020improving,wang2021admix,wang2023structure,xie2019improving,dong2019evading, lin2019nesterov}. This line of work seeks robust adversarial examples that provide consistent attack effects under various conditions.
2) Generating adversarial examples via simple geometric transformations~\cite{pei2017towards, engstrom2019exploring, xiao2018spatially, chen2020explore}. Without optimizing a $\ell_\infty$-norm bounded perturbation, this line of work optimizes transformation parameter, so that a slightly transformed image causes misprediction. While they provide new attacking form against deep networks through simple image transforms, the attacks are limited to certain transformation parameters and some requires to change the image semantic content~\cite{xiao2018spatially} or deviated from natural image color distribution~\cite{chen2020explore}, which limits their practicality.
In contrast, our work exploits the more general and diverse image transformations, covering spatial, photometric, and compression transformations to craft adversarial perturbations capable of dynamically altering their effects based on the transform applied. Introducing controllable attack effects by transforming the input in various ways.

% transfer attacks: \cite{xiaosen2023rethinking,wei2023enhancing,li2024improving}

% \Salnote{Anything on whitebox vs blackbox transfer attacks? If we have serious results on transfer success, we should add a subsection on that ... query-based transfer attacks ??? } \ytan{Re: we had a brief discussion of transfer attacks in section 2.1, since we are not proposing an transfer attack and not comapring with losts of (transfer/query-based) attacks, is this level of background discussion enough?}

==> figures/vis-cls.tex <==
\begin{figure*}[th]
\centering
%
% \vspace{-0.2cm}
% \begin{subfigure}[c]{0.95\linewidth}
%     \centering
    \includegraphics[width=1.0\textwidth]{figures/main/fig-cls.pdf}
% \end{subfigure}
\caption{We provide predictions for clean and perturbed (Adv.) images under each transformation with different parameters. For display, images under scaling are originally in resolutions of $\{112, 224, 336\}$ for $S\in\{0.5,1.0,1.5\}$ and are resized to $224$; the magnitude of residuals (i.e., $T(\mathbf{x};\theta)-T(\mathbf{x+\delta};\theta)$) and perturbations is amplified by $30\times$.}
\label{fig:cls}
\end{figure*}

==> tables/tab-cls-asr-eps10.tex <==
\begin{table*}[h]

\centering
\small
\caption{
Transformation-dependent targeted ASR (\%) $\uparrow$ of selected classification models. Higher value indicates better attack performance. The adversarial perturbation budget for this experiment is $\varepsilon=10$.
}
\label{tab:cls-asr}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transform\\ parameter\end{tabular}}} & \multicolumn{6}{c}{Classifier model} \\
\multicolumn{1}{c|}{} & VGG19 & ResNet50 & Dense121 & Incv3 & ViT-L-16 & ViT-L-32 \\ \hline
\multicolumn{7}{c}{Scaling} \\
\multicolumn{1}{c|}{$S=0.5$} & 99.50 & 96.80 & 95.60 & 76.70 & 77.60 & 61.70 \\
\multicolumn{1}{c|}{$S=1.0$} & 100.0 & 99.70 & 99.80 & 91.30 & 95.20 & 76.70 \\
\multicolumn{1}{c|}{$S=1.5$} & 100.0 & 99.60 & 99.60 & 84.00 & 91.60 & 71.80 \\ \hline
\multicolumn{1}{c|}{Average} & 99.83 & 98.70 & 98.33 & 84.00 & 88.07 & 70.07 \\ \hline
\multicolumn{7}{c}{Blurring} \\
\multicolumn{1}{c|}{$\sigma=0.5$} & 100.0 & 99.70 & 99.90 & 89.80 & 94.40 & 87.70 \\
\multicolumn{1}{c|}{$\sigma=1.5$} & 99.60 & 96.80 & 98.70 & 75.20 & 75.00 & 64.30 \\
\multicolumn{1}{c|}{$\sigma=3.0$} & 99.00 & 95.70 & 98.20 & 71.90 & 71.10 & 54.30 \\ \hline
\multicolumn{1}{c|}{Average} & 99.53 & 97.40 & 98.93 & 78.97 & 80.17 & 68.77 \\ \hline
\multicolumn{7}{c}{Gamma} \\
\multicolumn{1}{c|}{$\gamma=0.5$} & 100.0 & 99.90 & 99.80 & 89.40 & 95.30 & 89.50 \\
\multicolumn{1}{c|}{$\gamma=1.0$} & 100.0 & 99.90 & 100.0 & 91.70 & 97.90 & 92.40 \\
\multicolumn{1}{c|}{$\gamma=2.0$} & 100.0 & 99.80 & 99.90 & 88.50 & 87.80 & 77.50 \\ \hline
\multicolumn{1}{c|}{Average} & 100.0 & 99.87 & 99.90 & 89.87 & 93.67 & 86.47 \\ \hline
\multicolumn{7}{c}{JPEG} \\
\multicolumn{1}{c|}{$Q=20$} & 95.90 & 89.40 & 88.40 & 72.00 & 65.70 & 72.40 \\
\multicolumn{1}{c|}{$Q=50$} & 99.40 & 96.00 & 97.80 & 83.20 & 83.10 & 82.00 \\
\multicolumn{1}{c|}{$Q=80$} & 99.30 & 98.70 & 98.90 & 86.50 & 87.50 & 80.60 \\ \hline
\multicolumn{1}{c|}{Average} & 98.19 & 94.70 & 95.03 & 80.57 & 78.77 & 78.33 \\ \hline
\end{tabular}

\end{table*}

==> tables/tab-cls-asr.tex <==
\begin{table*}[h]

\centering
\small
\caption{
Transform-dependent targeted ASR (\%) $\uparrow$ of selected classification models. Higher value indicates better attack performance. The adversarial perturbation budget for this experiment is $\varepsilon=8$.
}
\label{tab:cls-asr}

\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transform\\ parameter\end{tabular}}} & \multicolumn{8}{c}{Classifier model} \\
\multicolumn{1}{c|}{}             & VGG19 & ResNet50 & Dense121 & Incv3 & Mobv2 & ViT-L-16 & ViT-L-32 & Swin-T \\ \hline
\multicolumn{9}{c}{Scaling}                                                                                  \\
\multicolumn{1}{c|}{$S=0.5$}      & 99.60 & 95.90    & 96.70    & 74.40 & 99.40 & 78.60   & 67.90   & 99.60  \\
\multicolumn{1}{c|}{$S=1.0$}      & 100.0 & 99.60    & 99.60    & 91.20 & 100.0 & 95.90   & 86.10   & 100.0  \\
\multicolumn{1}{c|}{$S=1.5$}      & 99.90 & 99.60    & 99.90    & 84.10 & 100.0 & 92.20   & 78.10   & 100.0  \\ \hline
\multicolumn{1}{c|}{Average}      & 99.83 & 98.37    & 98.73    & 83.23 & 99.80 & 88.90   & 77.37   & 99.87  \\ \hline
\multicolumn{9}{c}{Blurring}                                                                                 \\
\multicolumn{1}{c|}{$\sigma=0.5$} & 100.0 & 99.70    & 99.90    & 90.50 & 100.0 & 94.40   & 85.50   & 100.0  \\
\multicolumn{1}{c|}{$\sigma=1.5$} & 99.60 & 96.90    & 97.90    & 79.20 & 98.60 & 73.20   & 63.90   & 99.30  \\
\multicolumn{1}{c|}{$\sigma=3.0$} & 99.00 & 96.40    & 97.90    & 71.30 & 98.70 & 70.40   & 56.80   & 99.00  \\ \hline
\multicolumn{1}{c|}{Average}      & 99.53 & 97.67    & 98.57    & 80.33 & 99.10 & 79.33   & 68.73   & 99.43  \\ \hline
\multicolumn{9}{c}{Gamma}                                                                                    \\
\multicolumn{1}{c|}{$\gamma=0.5$} & 100.0 & 99.90    & 99.80    & 93.10 & 100.0 & 98.40   & 92.20   & 100.0  \\
\multicolumn{1}{c|}{$\gamma=1.0$} & 100.0 & 99.90    & 99.90    & 90.00 & 100.0 & 97.00   & 85.20   & 99.90  \\
\multicolumn{1}{c|}{$\gamma=2.0$} & 100.0 & 99.80    & 99.60    & 88.90 & 100.0 & 87.60   & 79.30   & 99.90  \\ \hline
\multicolumn{1}{c|}{Average}      & 100.0 & 99.87    & 99.77    & 90.67 & 100.0 & 94.33   & 85.57   & 99.93  \\ \hline
\multicolumn{9}{c}{JPEG}                                                                                     \\
\multicolumn{1}{c|}{$Q=20$}       & 96.10 & 89.20    & 92.80    & 73.20 & 95.60 & 70.60   & 71.70   & 84.10  \\
\multicolumn{1}{c|}{$Q=50$}       & 99.40 & 96.90    & 97.80    & 83.00 & 98.10 & 82.60   & 82.00   & 97.40  \\
\multicolumn{1}{c|}{$Q=80$}       & 99.70 & 98.50    & 99.10    & 86.80 & 99.80 & 88.60   & 81.30   & 99.30  \\ \hline
\multicolumn{1}{c|}{Average}      & 98.40 & 94.87    & 96.57    & 81.00 & 97.83 & 80.60   & 78.33   & 93.60  \\ \hline
\end{tabular}

\end{table*}

==> tables/tab-cls-blur.tex <==
\begin{table}[h]

\centering
\small

\caption{Blur-dependent targeted attack success rate (ASR). ASRs are reported at each target Gaussian blur standard deviation $\sigma$ and average over all three $\sigma$s.
Higher value indicates better attack performance. The perturbation budget is $\|\delta\|_\infty \leq 10$.
}
\label{tab:attack-blur}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Standard \\ deviation\end{tabular}}} & \multicolumn{6}{c}{Classifier model ASR (\%) $\uparrow$} \\
\multicolumn{1}{c|}{} & VGG-19 & ResNet-50 & Dense-161 & Inc-v3 & ViT-L-16 & ViT-L-32 \\ \hline
\multicolumn{1}{c|}{$\sigma=0.5$} & 100.0 & 99.70 & 99.90 & 89.80 & 94.40 & 87.70 \\
\multicolumn{1}{c|}{$\sigma=1.5$} & 99.60 & 96.80 & 98.70 & 75.20 & 75.00 & 64.30 \\
\multicolumn{1}{c|}{$\sigma=3.0$} & 99.00 & 95.70 & 98.20 & 71.90 & 71.10 & 54.30 \\ \hline
\multicolumn{1}{c|}{Average} & 99.53 & 97.40 & 98.93 & 78.97 & 80.17 & 68.77 \\ \hline
\end{tabular}

\end{table}

==> tables/tab-cls-gamma.tex <==
\begin{table*}[h]

\centering
\small
\caption{
ASR evaluation over selected classification models.
Higher value indicating lower classification error introduced by the image transformation.
}
\label{tab:cls-asr}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transform\\ parameter\end{tabular}}} & \multicolumn{6}{c}{Classifier model} \\
\multicolumn{1}{c|}{} & VGG19 & ResNet50 & Dense161 & Incv3 & ViT-L16 & ViT-L32 \\ \hline
\multicolumn{7}{c}{$T$: Scaling} \\
\multicolumn{1}{c|}{$0.5 \times$} & 99.50 & 96.80 & 95.60 & 76.70 & 77.60 & 61.70 \\
\multicolumn{1}{c|}{$1.0 \times$} & 100.0 & 99.70 & 99.80 & 91.30 & 95.20 & 76.70 \\
\multicolumn{1}{c|}{$1.5 \times$} & 100.0 & 99.60 & 99.60 & 84.00 & 91.60 & 71.80 \\ \hline
\multicolumn{1}{c|}{Average} & 99.83 & 98.70 & 98.33 & 84.00 & 88.07 & 70.07 \\ \hline
\multicolumn{7}{c}{$T$: Blurring} \\
\multicolumn{1}{c|}{$\sigma=0.5$} & 100.0 & 99.70 & 99.90 & 89.80 & 94.40 & 87.70 \\
\multicolumn{1}{c|}{$\sigma=1.5$} & 99.60 & 96.80 & 98.70 & 75.20 & 75.00 & 64.30 \\
\multicolumn{1}{c|}{$\sigma=3.0$} & 99.00 & 95.70 & 98.20 & 71.90 & 71.10 & 54.30 \\ \hline
\multicolumn{1}{c|}{Average} & 99.53 & 97.40 & 98.93 & 78.97 & 80.17 & 68.77 \\ \hline
\multicolumn{7}{c}{$T$: Gamma} \\
\multicolumn{1}{c|}{$\gamma=0.5$} & 100.0 & 99.90 & 99.80 & 89.40 & 95.30 & 89.50 \\
\multicolumn{1}{c|}{$\gamma=1.0$} & 100.0 & 99.90 & 100.0 & 91.70 & 97.90 & 92.40 \\
\multicolumn{1}{c|}{$\gamma=2.0$} & 100.0 & 99.80 & 99.90 & 88.50 & 87.80 & 77.50 \\ \hline
\multicolumn{1}{c|}{Average} & 100.0 & 99.87 & 99.90 & 89.87 & 93.67 & 86.47 \\ \hline
\multicolumn{7}{c}{$T$: JPEG} \\
\multicolumn{1}{c|}{$Q=20$} & 95.90 & 89.40 & 88.40 & 72.00 & 65.70 & 72.40 \\
\multicolumn{1}{c|}{$Q=50$} & 99.40 & 96.00 & 97.80 & 83.20 & 83.10 & 82.00 \\
\multicolumn{1}{c|}{$Q=80$} & 99.30 & 98.70 & 98.90 & 86.50 & 87.50 & 80.60 \\ \hline
\multicolumn{1}{c|}{Average} & 98.19 & 94.70 & 95.03 & 80.57 & 78.77 & 78.33 \\ \hline
\end{tabular}

\end{table*}

==> tables/tab-cls-jpeg.tex <==
\begin{table}[]

\centering
\small
\caption{Compression-dependent targeted attack success rate (ASR). ASRs are reported at each compression quality $Q$ and average over all three $Q$s.
Higher value indicates better attack performance. The perturbation budget is $\|\delta\|_\infty \leq 10$.

}
\label{tab:attack-jpeg}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression \\ quality\end{tabular}}} & \multicolumn{6}{c}{Classifier model ASR (\%) $\uparrow$} \\
\multicolumn{1}{c|}{} & VGG-19 & ResNet-50 & Dense-161 & Inc-v3 & ViT-L-16 & ViT-L-32 \\ \hline
\multicolumn{1}{c|}{$Q=20$} & 95.90 & 89.40 & 88.40 & 72.00 & 65.70 & 72.40 \\
\multicolumn{1}{c|}{$Q=50$} & 99.40 & 96.00 & 97.80 & 83.20 & 83.10 & 82.00 \\
\multicolumn{1}{c|}{$Q=80$} & 99.30 & 98.70 & 98.90 & 86.50 & 87.50& 80.60 \\ \hline
\multicolumn{1}{c|}{Average} & 98.19 & 94.70 & 95.03 & 80.57 & 78.77 & 78.33 \\ \hline
\end{tabular}

\end{table}

==> tables/tab-cls-rob.tex <==
\begin{table*}[]

\centering
\small
\caption{Results of attacking adversarial-robust models with transform-dependent attacks.
We use perturbation budget $\varepsilon=\{4,8\}$ for attacking \{ResNet50-eps4, ResNet50-eps8\} respectively. We report model consistency (\%) and ASR (\%) $\uparrow$ for adversarially perturbed images at \textit{Original} and \textit{Transformed} conditions respectively. Our attacks successfully lowered robust model consistency.
% \Salnote{Remove Resnet50 results and clean up the table/caption}
}
\label{tab:attack-rob}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{3}{c|}{Scaling} & \multicolumn{3}{c}{Blurring} \\ \cline{2-7} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Original} & \multicolumn{2}{c|}{Transformed} & \multicolumn{1}{c|}{Original} & \multicolumn{2}{c}{Transformed} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$S=1.0$} & $S=0.5$ & \multicolumn{1}{c|}{$S=1.5$} & \multicolumn{1}{c|}{(no blur)} & $\sigma=0.5$ & $\sigma=1.5$ \\ \hline
% \multicolumn{1}{c|}{ResNet50} & \multicolumn{1}{c|}{94.00} & 99.67 & \multicolumn{1}{c|}{100.0} & \multicolumn{1}{c|}{0.0} & 100.0 & 99.67 \\
\multicolumn{1}{c|}{ResNet50-eps4} & \multicolumn{1}{c|}{87.67} & 67.33 & \multicolumn{1}{c|}{53.17} & \multicolumn{1}{c|}{76.00} & 29.33 & 57.67 \\
\multicolumn{1}{c|}{ResNet50-eps8} & \multicolumn{1}{c|}{82.00} & 79.00 & \multicolumn{1}{c|}{49.00} & \multicolumn{1}{c|}{65.00} & 40.00 & 61.67 \\ \hline
\multicolumn{1}{c|}{Average} & \multicolumn{1}{c|}{84.84} & 73.17 & \multicolumn{1}{c|}{51.09} & \multicolumn{1}{c|}{70.50} & 34.67 & 59.67 \\ \hline
\multicolumn{7}{l}{} \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{3}{c|}{Gamma correction} & \multicolumn{3}{c}{JPEG compression} \\ \cline{2-7} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Original} & \multicolumn{2}{c|}{Transformed} & \multicolumn{1}{c|}{Original} & \multicolumn{2}{c}{Transformed} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\gamma=1.0$} & $\gamma=0.5$ & \multicolumn{1}{c|}{$\gamma=2.0$} & \multicolumn{1}{c|}{$Q=100$} & $Q=50$ & $Q=80$ \\ \hline
% \multicolumn{1}{c|}{ResNet50} & \multicolumn{1}{c|}{9.00} & 100.0 & \multicolumn{1}{c|}{100.0} & \multicolumn{1}{c|}{74.37} & 98.67 & 99.67 \\
\multicolumn{1}{c|}{ResNet50-eps4} & \multicolumn{1}{c|}{99.33} & 61.67 & \multicolumn{1}{c|}{69.33} & \multicolumn{1}{c|}{81.67} & 48.67 & 46.67 \\
\multicolumn{1}{c|}{ResNet50-eps8} & \multicolumn{1}{c|}{99.33} & 66.00 & \multicolumn{1}{c|}{75.00} & \multicolumn{1}{c|}{75.00} & 52.33 & 50.78 \\ \hline
\multicolumn{1}{c|}{Average} & \multicolumn{1}{c|}{99.33} & 63.84 & \multicolumn{1}{c|}{72.17} & \multicolumn{1}{c|}{78.34} & 50.50 & 48.73 \\ \hline
\end{tabular}

% \vspace{-4mm}

\end{table*}

==> tables/tab-cls-scale.tex <==
\begin{table}[h]

\centering
\small
\caption{Scale-dependent targeted attack success rate (ASR). ASRs are reported at each target scaling factor and average over all three factors.
Higher value indicates better attack performance.
Perturbation budget is $\|\delta\|_\infty \leq 10$.
}
\label{tab:attack-scale}

\begin{tabular}{ccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Scaling \\ factor\end{tabular}}} & \multicolumn{6}{c}{Classifier model ASR (\%) $\uparrow$} \\
\multicolumn{1}{c|}{} & VGG-19 & ResNet-50 & Dense-161 & Inc-v3 & ViT-L-16 & ViT-L-32 \\ \hline
\multicolumn{1}{c|}{$0.5 \times$} & 99.50 & 96.80 & 95.60 & 76.70 & 77.60 & 61.70 \\
\multicolumn{1}{c|}{$1.0 \times$} & 100.0 & 99.70 & 99.80 & 91.30 & 95.20 & 76.70 \\
\multicolumn{1}{c|}{$1.5 \times$} & 100.0 & 99.60 & 99.60 & 84.00 & 91.60 & 71.80 \\ \hline
\multicolumn{1}{c|}{Average} & 99.83 & 98.70 & 98.33 & 84.00 & 88.07 & 70.07 \\ \hline
\end{tabular}

\end{table}
